Predicate Subtypes in VerCors

Predicate subtypes provide an attractive mechanism to specify range constraints on variable declarations. This paper discusses how we add support for predicate subtypes to the VerCors program verifier. Our approach automatically generates appropriate specifications from predicate subtype declarations. It provides support to easily combine multiple subtypes for a single variable declaration. Moreover, in order to use predicate subtypes for overflow checking, a special strict mode is introduced, where every subexpression also has to stay within the declared subtype. A prototype implementation is integrated into the VerCors verifier.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{Lorenzo Gheri \& Kirstin Peters (Eds.): 17th International\\ Workshop on Programming Language Approaches to Concurrency\\ and Communication-cEntric Software 2026 (PLACES 2026)\\
EPTCS 444, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.444.6}{10.4204/EPTCS.444.6}}
\pdfoutput=1

